Sketching Linear Classifiers over Data Streams

We introduce a new sub-linear space sketch---the Weight-Median Sketch---for learning compressed linear classifiers over data streams while supporting the efficient recovery of large-magnitude weights in the model. This enables memory-limited execution of several statistical analyses over streams, including online feature selection, streaming data explanation, relative deltoid detection, and streaming estimation of pointwise mutual information. Unlike related sketches that capture the most frequently-occurring features (or items) in a data stream, the Weight-Median Sketch captures the features that are most discriminative of one stream (or class) compared to another. The Weight-Median Sketch adopts the core data structure used in the Count-Sketch, but, instead of sketching counts, it captures sketched gradient updates to the model parameters. We provide a theoretical analysis that establishes recovery guarantees for batch and online learning, and demonstrate empirical improvements in memory-accuracy trade-offs over alternative memory-budgeted methods, including count-based sketches and feature hashing.

==> old_corollary.tex <==
\subsection{Corollary \ref{cor:stochastic}}

In the stochastic setting, we assume that a point is drawn uniformly at random from the $T$ data points for each of the $T$ time steps. Let $f_t(w)$ be the loss function corresponding to the data point chosen in the $t$th time step. Note that $\E[f_t(w)]=\hat{J}(w)$. Let $\hat{w}_t$ be the weight vector at the $t$th time step for online updates on the projected problem. Let $\hat{w}_{ol}=\frac{1}{N}\sum_{i=1}^{N}\hat{w}_i$ be the average of the weight vectors for all the $N$ time steps. We claim that $\hat{w}_{ol}$ is good with respect to $\hat{w}_{*}$, the optimizer of $\hat{J}(w)$. By the definition of regret,
\begin{align*}
\text{Regret}(\hat{w}_{*}) = \sum_{t=1}^{T}[f_t(\hat{w}_t)-f_t(\hat{w}_*)]
\end{align*}
Averaging by $T$ and taking expectations,
\begin{align}
\E\Big[\sum_{t=1}^{T}f_t(\hat{w}^t) \Big] \le \E\Big[\sum_{t=1}^{T}f_t(\hat{w}_*) \Big] +\frac{\E[\text{Regret}(\hat{w}_{*})]}{T} \label{eq:sgd1}
\end{align}
By Jensen's inequality and convexity of $\hat{J}(w)$,
\[
\hat{J}(\hat{w}_{ol}) \le \frac{1}{T}\sum_{i=1}^{T}\hat{J}(\hat{w}_{t})
\]
Therefore taking expectations and using the fact that $\hat{J}(w)=\E[f_t(w)]$,
\begin{align*}
\E[\hat{J}(\hat{w}_{ol})] \le \E\Big[\frac{1}{T}\sum_{i=1}^{T}\hat{J}(\hat{w}_{t})\Big]=\E\Big[\frac{1}{T}\sum_{i=1}^{T}f_t(\hat{w}_{t})\Big]
\end{align*}
Also, as $\hat{J}(w)=\E[f_t(w)]$,
\[
\hat{J}(\hat{w}_*)=\E\Big[\frac{1}{T}\sum_{i=1}^{T}f_t(\hat{w}_{*})\Big]
\]
Now using Eq. \ref{eq:sgd1},
\begin{align}
\E[\hat{J}(\hat{w}_{ol})] \le \hat{J}(\hat{w}_*) +\frac{\E[\text{Regret}(\hat{w}_{*})]}{T} \label{eq:sgd_regret}
\end{align}
By standard regret bounds on online gradient descent,
\begin{align}
\sum_{t=1}^{T}f_t(\hat{w}_t) \le \min_{w:\norm{w}\le \norm{w_*}} \sum_{t=1}^{T}f_t(w)+G\sqrt{T}\norm{w_*}\label{eq:sgd2}
\end{align}
As $\min_{w:\norm{w}\le \norm{w_*}} \sum_{t=1}^{T}f_t(w) \le \sum_{t=1}^{T}f_t(\hat{w}_*)$, using Eq. \ref{eq:sgd2} and the definition of $\text{Regret}(\hat{w}_{*})$,
\[
\text{Regret}(\hat{w}_{*})\le G\sqrt{T}\norm{w_*}
\]
Plugging this in Eq. \ref{eq:sgd_regret},
\begin{align}
\E[\hat{J}(\hat{w}_{ol})] \le \hat{J}(\hat{w}_*) +{G\norm{w_*}}/{\sqrt{T}} \label{eq:sgd_bnd}
\end{align}
We will now bound the expected distance between $\hat{w}_{ol}$ and $\hat{w}_*$ using Eq. \ref{eq:sgd_bnd} the strong convexity of $\hat{J}(w)$. Note that $\hat{J}(w)$ is $\lambda$ strong-convex (as $\hat{J}(w-\frac{\lambda}{2}\normsq{w})$ is convex) and $\nabla\hat{J}(\hat{w}_*)=0$  (as $\hat{w}_*$ is the minimizer of $\hat{J}(w)$). Therefore, 
\begin{align*}
&\hat{J}(\hat{w}_*) + \frac{\lambda}{2}\normsq{\hat{w}_{ol}-\hat{w}_*}\le \hat{J}(\hat{w}_{ol})\\
\implies &\normsq{\hat{w}_{ol}-\hat{w}_*} \le \frac{2}{\lambda}[\hat{J}(\hat{w}_{ol})-\hat{J}(\hat{w}_*)]\\
\implies &\E\Big[\normsq{\hat{w}_{ol}-\hat{w}_*}\Big] \le \frac{2}{\lambda}\Big[\E[\hat{J}(\hat{w}_{ol})]-\hat{J}(\hat{w}_*)\Big]
\end{align*}
Using Eq. \ref{eq:sgd_bnd} and then Jensen's inequality,
\begin{align}
\E\Big[\norm{\hat{w}_{ol}-\hat{w}_*}\Big] \le \frac{2G\norm{w_*}}{\lambda\sqrt{T}} \label{eq:sgd_edist}
\end{align}
Let $\hat{w}_{ol-cs}=\sqrt{s}\hat{w}_{ol}$. Let $\hat{w}_{ol-est}$ be the count-sketch estimate of $w_*$ derived from $\hat{w}_{ol-cs}$. Following the same argument as in the proof of Theorem \ref{thm:batch-recovery}, 
\begin{align*}
\lpnorm{\hat{w}_{est}-\hat{w}_{ol-est}}{\infty}&\le\lpnorm{\hat{w}_{cs}-\hat{w}_{ol-cs}}{\infty}\\
&\le \norm{\hat{w}_{cs}-\hat{w}_{ol-cs}}\\
&= \sqrt{s}\norm{\hat{w}_{*}-\hat{w}_{ol}}
\end{align*}
Therefore, using Eq. \ref{eq:sgd_edist}, 
\begin{align}
\E[\lpnorm{\hat{w}_{est}-\hat{w}_{ol-est}}{\infty}] \le \frac{2G\norm{w_*}}{\lambda}\sqrt{\frac{s}{T}}
\end{align}
By triangle inequality, 
\begin{align}
&\lpnorm{w_*-\hat{w}_{ol-est}}{\infty}\le \lpnorm{w_*-\hat{w}_{est}}{\infty}+\lpnorm{\hat{w}_{est}-\hat{w}_{ol-est}}{\infty}\nonumber\\
\implies &\E\Big[\lpnorm{w_*-\hat{w}_{ol-est}}{\infty}\Big]\le \E\Big[\lpnorm{w_*-\hat{w}_{est}}{\infty}\Big]+\E\Big[\lpnorm{\hat{w}_{est}-\hat{w}_{ol-est}}{\infty}\Big]\nonumber
\end{align}
By Theorem \ref{thm:batch-recovery}, for fixed constants $C',C''$ and 
\begin{align*}
k= {(C'/\epsilon^4)\log^3(d/\delta)\max\{1,L^2R^4/\lambda^2\}}\\
s={(C''/\epsilon^2)\log^2(d/\delta)\max\{1,LR^2/\lambda\}}
\end{align*}
with probability $1-\delta$,
\[
\lpnorm{w_*-\hat{w}_{est}}{\infty} \le \epsilon \| w_* \|_1
\]
Therefore, for slightly larger constants $C'$ and $C''$, with probability $1-\delta$,
\[
\E\Big[\lpnorm{w_*-\hat{w}_{ol-est}}{\infty}\Big] \le \frac{\epsilon}{2}\lpnorm{w_*}{1} + \sqrt{\frac{4C''G^2\log^2(d/\delta)\max\{1,LR^2/\lambda\}}{\epsilon^2T}}\norm{w_*}
\]
Therefore for $T\ge (C'''/(\epsilon^4\lambda^2))G^2\log^2(d/\delta)\max\{1,LR^2/\lambda\}$,
\[
\E\Big[\lpnorm{w_*-\hat{w}_{ol-est}}{\infty}\Big] \le \frac{\epsilon}{2}\lpnorm{w_*}{1} +\frac{\epsilon}{2}\lpnorm{w_*}{2} \le {\epsilon}\lpnorm{w_*}{1}
\]



==> proofs.tex <==
\section{Proofs}
\subsection{Proof of Theorem \ref{thm:batch-recovery}}\label{sec:proofs}
% \section{Introduction}

\iffalse
Consider a loss function $\ell(z)$ which is convex and $L$-strongly smooth. Suppose our goal is to minimize the total loss over all training points $\b{x}_i \in \mathbb{R}^d, i \in [n]$, subject to regularization ---
\begin{align*}
    J(w) &= \frac{1}{T}\sum_i \ell(y_iw^Tx_i) + \frac{\lambda}{2}\normsq{w}
\end{align*} 
 Similarly, let $\hat{J}(w)$ be the objective function obtained by projecting each point $\b{x}_i$ to ${R}x_i$ using the projection matrix ${R}\in \mathbb{R}^{k \times d}$ ---
\begin{align*}
    \hat{J}(w) &= \frac{1}{T}\sum_i \ell(y_iw^T({R}x_i)) + \frac{\lambda}{2}\normsq{w}
\end{align*}
Recall that ${R}$ is the sparse JL matrix in \citet{kane2014sparser} which has a fixed number $s$ of non-zero entries per column. We show that under appropriate values of the projection dimension $d$ and the sparsity $s$, we can accurately recover a good approximation to the minimizer of the original objective function.
\fi


We will use the duals of $L(\b{w})$ and $\hat{L}(\b{z})$ to show that $\b{z}_*$ is close to $R \b{w}_*$, following the analysis of \citet{zhang2014random} and \citet{yang2015theory}. Define ${\tilde{\mathbf{x}}}_i = y_i \b{x}_i$, i.e. the $i$th data point $\b{x}_i$ times its label. Let ${\tilde{X}}\in \mathbb{R}^{d \times T}$ be the matrix of data points such that the $i$th column is $\mathbf{\tilde{x}}_i$. Let ${G}={\tilde{X}}^T{\tilde{X}}$ be the Gram matrix corresponding to the original data points. Forming the Lagrangian and minimizing with respect to the primal variables gives us the following dual objective function in terms of the dual variable $\mathbf{\alpha} \in \mathbb{R}^T$,
\begin{align*}
J(\mathbf{\alpha}) &= \frac{1}{T}\sum_i \ell^*(\b{\alpha}_i) + \frac{1}{2\lambda T^2}\b{\alpha}^T {G} \b{\alpha},
\end{align*}
where $\ell^*(\b{\alpha}_i)$ is the Fenchel conjugate of $\ell(z_i)$. Note that if $\b{\alpha}_*$ is the minimizer of $J(\b{\alpha})$, then the minimizer $\b{w}_*$ of $L(\b{w})$ is given by $\b{w}_* = -\frac{1}{\lambda T} {\tilde{X}} \b{\alpha}_*$.

We similarly define ${G}={\tilde{X}}^T{R}^T{R}{\tilde{X}}$ as the Gram matrix corresponding to the projected data points. We can write down the dual $\hat{L}(\b{\alpha})$ of the projected primal objective function $\hat{J}(\b{w})$  in terms of the dual variable $\hat{\b{\alpha}}$ as follows:
\begin{align*}
\hat{J}(\hat{\b{\alpha}}) &= \frac{1}{T}\sum_i \ell^*(\hat{\b{\alpha}}_i) + \frac{1}{2\lambda T^2}\hat{\b{\alpha}}^T \hat{{G}} \hat{\b{\alpha}}.
\end{align*}
As before, if $\hat{\b{\alpha}}_*$ is the minimizer of $ \hat{J}(\hat{\b{\alpha}})$, then the minimizer $\b{z}_*$ of $\hat{L}(\b{z})$ is given by $\hat{\b{w}}_* = -\frac{1}{\lambda T} {R}\tilde{X} \hat{\b{\alpha}}_*$.

We will first express the distance between $\b{z}_*$ and ${R}\b{w}_*$ in terms of the distance between the dual variables. We can write:
\begin{align}
\normsq{\b{z}_*-{R}\b{w}_*} &= \frac{1}{\lambda^2T^2} \normsq{{R}\tilde{X}\hat{\b{\alpha}}_*-{R}\tilde{X}\b{\alpha}_*}\nonumber\\
&= \frac{1}{\lambda^2T^2} (\hat{\b{\alpha}}_*-\b{\alpha}_*)^T \hat{{G}} (\hat{\b{\alpha}}_*-\b{\alpha}_*).\label{eq:relate1}
\end{align}
Hence, our goal will be to upper bound $(\hat{\b{\alpha}}_*-\b{\alpha}_*)^T \hat{{G}} (\hat{\b{\alpha}}_*-\b{\alpha}_*)$. Define $\b{\Delta} = \frac{1}{\lambda T}(\hat{{G}}-{G}) \b{\alpha}_*$. We will show that 
$(\hat{\b{\alpha}}_*-\b{\alpha}_*)^T \hat{{G}} (\hat{\b{\alpha}}_*-\b{\alpha}_*)$ can be upper bounded in terms of $\b{\Delta}$ as follows. 
\begin{lemma}\label{lemma:delta}
	\begin{align*}
	\frac{1}{\lambda^2 T^2}(\hat{\b{\alpha}}_*-\b{\alpha}_*)^T \hat{{G}} (\hat{\b{\alpha}}_*-\b{\alpha}_*) &\le  \frac{2\beta}{\lambda} \| \b{\Delta} \|_{\infty}^2
	\end{align*}
\end{lemma}
Due to space constraints, we omit the proof of Lemma \ref{lemma:delta} here, deferring it to the full version of the paper. The proof relies on the convexity and strong-smoothness of the loss function $\ell$. 

We now bound $\| \b{\Delta}\|_{\infty}$. The result relies on the JL property of the projection matrix ${R}$ (recall Definition \ref{def:JL}). If ${R}$ is a JL matrix with error $\epsilon$ and failure probability $\delta/d^2$, then it is straightforward to verify that with failure probability $\delta$, for all coordinate basis vectors $\{\b{e}_1, \dots, \b{e}_d\}$,
\begin{align}
\norm{{R}\b{e}_i} = 1 \pm \epsilon,\; \forall \; i, \quad  |\langle {R}\b{e}_i, {R}\b{e}_j \rangle | \le \epsilon, \; \forall \; i \ne j.\label{eq:ip_preserve}
\end{align}
\iffalse
The first bound follows directly from the JL property, to derive the bound on the inner product, we rewrite the inner product as follows,
\begin{align*}
4\langle {R}\b{e}_i, {R}\b{e}_j \rangle = \normsq{{R}\b{e}_i+{R}\b{e}_j}-\normsq{{R}\b{e}_i-{R}\b{e}_j}
\end{align*}
The bound then follows by using the JL property for $\normsq{{R}\b{e}_i+{R}\b{e}_j}$ and $\normsq{{R}\b{e}_i-{R}\b{e}_j}$. As there are $d^2$ pairs, if the inner product is preserved for each pair with failure probability $\delta/d^2$, then by a union bound it is preserved simultaneously for all of them with failure probability $\delta$.
\fi
Using this projection, we show the following bound on $\|\b{\Delta}\|_\infty$:
\begin{lemma}\label{lemma:bound_delta}
     If ${R}$ satisfies condition \ref{eq:ip_preserve}, then:
    \[
    \|\b{\Delta}\|_{\infty}\le 2\gamma\epsilon \| \b{w}_* \|_1,
    \]
    where $\gamma= \max_i \|\b{x}_i\|_1$.
\end{lemma}
\begin{proof}
	We first rewrite $\b{\Delta}$ as follows,
	\begin{align*}
	\b{\Delta}& = \frac{1}{\lambda T} (\tilde{X}^T{R}^T{R}\tilde{X}-\tilde{X}^T\tilde{X})\b{\alpha}_*=\frac{1}{\lambda T} \tilde{X}^T({R}^T{R}-{I})\tilde{X}\b{\alpha}_*\\
	&= \tilde{X}^T({I}-{R}^T{R})\b{w}_*,
	\end{align*}
	using the relation that $\b{w}_* = -\frac{1}{\lambda T}\tilde{X}\b{\alpha}_*$. Therefore,
	\[
	\lpnorm{\b{\Delta}}{\infty} \le \max_i | \b{x}_i^T({I}-{R}^T{R})\b{w}_* | = \max_i | \b{x}_i^T\b{w}_*-({R}\b{x}_i)^T({R}\b{w}_*) |.
	\]
	We now claim that if condition \ref{eq:ip_preserve} is satisfied, then for any two vectors $\b{v}_1$ and $\b{v}_2$, 
	\begin{align}
	|\b{v}_1^T\b{v}_2 - ({R}\b{v}_1)^T({R}\b{v}_2)| \le 2\epsilon \lpnorm{\b{v}_1}{1}\lpnorm{\b{v}_2}{1}.\label{eq:jl_l1}
	\end{align}
The proof follows from simple algebra, and is omitted from this version for lack of space. Using this relation, it follows that,
\[
\lpnorm{\b{\Delta}}{\infty} \le \max_i | \b{x}_i^T\b{w}_*-({R}\b{x}_i)^T({R}\b{w}_*) | \le 2\epsilon \gamma \lonenorm{\b{w}_*}.
\]
\end{proof}	
%\begin{lemma}\label{lemma:bound_delta}
%    \citep{yang2015theory} If ${R}$ is a JJ matrix with error $\epsilon$ and failure probability $\delta/n$, then with probability $1-2\delta$, we have,
%    \[
%    \|\b{\Delta}\|_{\infty}\le R \| \b{w}_* \|_2 \epsilon_{{R},\delta/n}
%    \]
%    where $R = \max_i \|\b{x}_i\|_2$
%\end{lemma}

We will now combine Lemma \ref{lemma:delta} and \ref{lemma:bound_delta}. By Eq. \ref{eq:relate1} and Lemma \ref{lemma:delta},
\[
\normsq{\b{z}_*-{R}\b{w}_*} \le  \frac{2\beta}{\lambda }  \| \b{\Delta} \|_{\infty}^2.
\]
If ${R}$ is a JL matrix with error $\epsilon$ and failure probability $\delta/d^2$, then by Lemma \ref{lemma:bound_delta}, with failure probability $\delta$,
\begin{align}
\norm{\b{z}_*-{R}\b{w}_*} \le 4\gamma\epsilon\sqrt{\frac{\beta}{\lambda}} \| \b{w}_* \|_1.  \label{eq:e1}
\end{align}
By \citet{kane2014sparser}, the random projection matrix ${R}$ satisfies the JL property with error $\theta$ and failure probability $\delta'/d^2$ for $k\ge{C\log(d/\delta')/\theta^2}$, where $C$ is a fixed constant. Using Eq. \ref{eq:e1}, with failure probability $\delta'$,
\begin{align}
\norm{\b{z}_*-{R}\b{w}_*} \le 4\gamma\theta\sqrt{\frac{\beta}{\lambda}} \| \b{w}_* \|_1.  \label{eq:e2}
%\norm{\b{z}_*-{R}\b{w}_*} \le \sqrt{\frac{2J}{\lambda}}R \| \b{w}_* \|_2 \theta\label{eq:e2}
%\| \b{w}_* \|_2\sqrt{\frac{2JC\gamma^2\log(n/\delta)}{\lambda k}}
\end{align}
Recall that $\sqrt{s}R$ is a Count-Sketch matrix with width $C_1/\theta$ and depth $s=C_2\log(d/\delta')/\theta$, where $C_1$ and $C_2$ are fixed constants. Let $\b{w}_{\mathrm{proj}}$ be the projection of $\b{w}_*$ with the Count-Sketch matrix $\tilde{{R}}$, hence $\b{w}_{\mathrm{proj}}=\sqrt{s}{R}\b{w}_*$. Let $\b{z}_{\mathrm{proj}}=\sqrt{s}\b{z}_*$. By Eq. \ref{eq:e2}, with failure probability $\delta'$,
\[
\norm{\b{z}_{\mathrm{proj}}-\b{w}_{\mathrm{proj}}} \le \sqrt{\frac{16\beta \gamma^2\theta\log(d/\delta')}{\lambda}}\| \b{w}_* \|_1.
\]
Let $\b{w}_{\mathrm{cs}}$ be the Count-Sketch estimate of $\b{w}_*$ derived from $\b{w}_{\mathrm{proj}}$, and $\b{w}_{\mathrm{est}}$ be the Count-Sketch estimate of $\b{w}_*$ derived from $\b{z}_{\mathrm{proj}}$. Recall that the Count-Sketch estimate of a vector is the median of the estimates of all the locations to which the vector hashes. As the difference between the median of any two vectors is at most the $\ell_{\infty}$-norm of their difference,
\begin{align*}
\lpnorm{\b{w}_{\mathrm{est}}-\b{w}_{\mathrm{cs}}}{\infty}\le \lpnorm{\b{z}_{\mathrm{proj}}-\b{w}_{\mathrm{proj}}}{\infty}.
\end{align*}
Therefore with failure probability $\delta'$,
\begin{align}
\lpnorm{\b{w}_{\mathrm{est}}-\b{w}_{\mathrm{cs}}}{\infty}\le \lpnorm{\b{z}_{\mathrm{proj}}-\b{w}_{\mathrm{proj}}}{\infty}\le  \norm{\b{z}_{\mathrm{proj}}-\b{w}_{\mathrm{proj}}}\nonumber\\
 \le \sqrt{\frac{16\beta \gamma^2\theta\log(d/\delta')}{\lambda}}\| \b{w}_* \|_1. \label{eq:e3}
\end{align}
We now use Lemma \ref{lem:count-sketch} to bound the error for Count-Sketch recovery. Using Lemma \ref{lem:count-sketch} for the  matrix $\sqrt{s}{{R}}$, with failure probability $\delta'$,
\[
\lpnorm{\b{w}_*-\b{w}_{\mathrm{cs}}}{\infty} \le \sqrt{\theta} \norm{\b{w}_*}.
\]
Now using the triangle inequality and Eq. \ref{eq:e3}, with failure probability $2\delta'$ (due to a union bound),
\begin{align*}
\lpnorm{\b{w}_*-\b{w}_{\mathrm{est}}}{\infty}&\le \lpnorm{\b{w}_*-\b{w}_{\mathrm{est}}}{\infty}+\lpnorm{\b{w}_{\mathrm{est}}-\b{w}_{\mathrm{cs}}}{\infty}\\
&\le \sqrt{\theta} \norm{\b{w}_*} + \sqrt{\frac{16\beta \gamma^2\theta\log(d/\delta')}{\lambda}}\| \b{w}_* \|_1\\
&\le \left( \sqrt{\theta} + \sqrt{\frac{16\beta \gamma^2\theta\log(d/\delta')}{\lambda}}\right)\| \b{w}_* \|_1.
\end{align*}
Therefore choosing $\theta = \min\{1,\lambda / (16\beta \gamma^2\log(d/\delta'))\}\epsilon^2/4$, with failure probability $2\delta'$,
\[
\lpnorm{\b{w}_*-\b{w}_{\mathrm{est}}}{\infty} \le \epsilon \| \b{w}_* \|_1.
\]
Choosing $\delta'=\delta/2$,
%$k= {(C_1/\epsilon^4)\log^3(d/\delta)\max\{1,\beta^2\gamma^4/\lambda^2\}}$, and $s={(C_2/\epsilon^2)\log^2(d/\delta)\max\{1,\beta\gamma^2/\lambda\}}$
we have that for fixed constants $C_1,C_2$,
\begin{align*}
k&= {(C_1/\epsilon^4)\log^3(d/\delta)\max\{1,\beta^2\gamma^4/\lambda^2\}},\\
s&={(C_2/\epsilon^2)\log^2(d/\delta)\max\{1,\beta\gamma^2/\lambda\}},
\end{align*}
$\lpnorm{\b{w}_*-\b{w}_{\mathrm{est}}}{\infty} \le \epsilon \| \b{w}_* \|_1$, with probability $1-\delta$.
%\input{proofs_full}
\input{new_corollary}
%\input{sketch-appendix}
\input{baseline}


==> related-work.tex <==
\section{Related Work}
\label{sec:related}

%\pb{Note that this is really, really heavy on ML. Can you devote more space to work appearing in SIGMOD and VLDB? This seems a little silly, but you don't want database people to wonder why you sent this to SIGMOD (e.g., is this an ICML rejection?)...}

\minihead{Heavy-Hitters in Data Streams} The Heavy-Hitters problem has been extensively studied in the 
streaming algorithms literature. Given a sequence of items, the goal is to return the set of all items whose frequency exceeds a specified
fraction of the total number of items. Algorithms for finding frequent items can be broadly categorized into counter-based approaches \citep{manku2002approximate,demaine2002frequency,karp2003simple,metwally2005efficient}, quantile algorithms 
\citep{greenwald2001space,shrivastava2004medians}, and sketch-based methods \citep{charikar2002finding,cormode2005improved}.
 
Mirylenka et al. \citep{mirylenka2015conditional} develop streaming algorithms for finding \emph{conditional} heavy-hitters, where the goal is to identify items that are frequent in the context of a separate ``parent'' item. While these methods can be used in related applications to ours, their counter-based algorithms differ significantly from our classification-based approach.

\minihead{Characterizing Changes in Data Streams} The problem of detecting and characterizing significant absolute and relative differences between data streams has been studied by several authors. \citet{cormode2005s} proposed a Count-Min-based algorithm for identifying items whose occurrence rates differ significantly; \citet{schweller2004reversible} propose reversible hashes in this context to avoid storing key information. These approaches focus primarily on identifying differences between time periods, whereas we focus on the case where streams are observed concurrently. In order to explain anomalous traffic flows, \citet{brauckhoff2012anomaly} proposed techniques using histogram-based detectors and association rules. Using histograms to identify changes in feature occurrence is appropriate for detecting large absolute differences; in contrast, we focus on detecting relative differences, a problem which has previously been found to be challenging \citep{cormode2005s}.

%\pbnote{Have a separate para on relative deltoids! also cite and compare to sketches for ``change detection'', reversible sketches, reverse hashing \url{https://scholar.google.com/scholar?cites=1847512584342634183&as_sdt=2005&sciodt=0,5&hl=en}; here is one way a reviewer can kill your paper: ``oh, doesn't cite X, which SOUNDS similar'' -- you will get less credit for the stuff below here.}

\minihead{Resource-Efficient ML} \citet{gupta2017protonn} and \citet{kumar2017resource} explore the use of tree- and $k$-nearest-neighbor-based classifiers on highly resource-constrained devices. A large body of work studies resource-efficient inference at test time \citep{xu2012greedy,xu2013cost,hsieh2014fast}. Unlike budget kernel methods \citep{crammer2004online} that maintain a small set of support vectors, we aim to directly restrict the number of parameters stored. Our work also differs from \emph{model compression} or \emph{distillation}, which aims to imitate a large, expensive model using a smaller one with lower memory and computation costs \citep{bucilu?2006model,ba2014deep,hinton2015distilling}.

\minihead{Sparsity-Inducing Regularization} $\ell_1$-regularization is a standard technique for encouraging parameter sparsity in online learning \citep{langford2009sparse,duchi2009efficient,xiao2010dual,mcmahan2011follow}. In practice, it is difficult to \emph{a priori} select an $\ell_1$ regularization strength in order to satisfy a given sparsity budget; it can therefore be problematic to apply standard online learning methods in settings with hard memory constraints. In this paper, we propose a different approach: we first fix a memory budget and then use the allocated space to approximate a classifier, with the property that our approximation will be better for parameter vectors with small $\ell_1$-norm (see Theorem~\ref{thm:online}). We note that the WM-Sketch and AWM-Sketch are compatible with the use of an $\ell_1$-regularizer in addition to the requisite $\ell_2$ term.

% In online learning, an $\ell_1$-penalized objective $\ell(\mathbf{w}) + \lambda_1 \|\mathbf{w}\|_1$ is typically optimized using an online convex optimization algorithm that has been shown empirically to be effective at inducing sparsity. Examples of such algorithms include Truncated Gradient \citep{langford2009sparse}, Forward-Backward Splitting \citep{duchi2009efficient}, Regularized Dual Averaging \citep{xiao2010dual}, and FTRL-Proximal \citep{mcmahan2011follow}. 

% In a separate line of work, Bahmani et al. \citep{bahmani2013greedy} consider the problem of learning linear models under L0 constraints; however, their work focuses on the batch setting, whereas we focus on online learning with streaming updates.

\minihead{Feature Hashing} Feature hashing \citep{shi2009hash,weinberger2009feature} is a technique where the classifier is trained on features that have been hashed to a fixed-width table. This approach lowers memory usage by reducing the dimension of the feature space and by obviating the need for storing feature identifiers, but at the cost of model interpretability.
 
\minihead{Compressed Learning} Calderbank et al. \citep{calderbankcompressed} introduced \emph{compressed learning}, where a classifier is trained on data obtained via compressive sensing \citep{candes2006near,donoho2006compressed}. The authors focus on classification performance in the compressed domain and do not consider the problem of recovering weights in the original space.

